Characterizing the universal rigidity of generic frameworks

A framework is a graph and a map from its vertices to E^d (for some d). A framework is universally rigid if any framework in any dimension with the same graph and edge lengths is a Euclidean image of it. We show that a generic universally rigid framework has a positive semi-definite stress matrix of maximal rank. Connelly showed that the existence of such a positive semi-definite stress matrix is sufficient for universal rigidity, so this provides a characterization of universal rigidity for generic frameworks. We also extend our argument to give a new result on the genericity of strict complementarity in semidefinite programming.

==> Makefile <==
MAIN = UniversalRigidity
TEXSOURCES = $(MAIN).tex defs.tex macros.tex intro.tex measurement.tex \
	convex.tex sdp.tex
BIBFILES = graphs.bib convex.bib
LATEX = latex
PDFLATEX = pdflatex

all: $(MAIN).pdf

check: figures-stamp
	$(LATEX) $(MAIN)
	$(PDFLATEX) $(MAIN)
	bibtex $(MAIN)

$(MAIN).pdf: $(TEXSOURCES) $(COMMONFILES) figures-stamp
	$(PDFLATEX) $(MAIN)
	bibtex $(MAIN)
	$(PDFLATEX) $(MAIN)
	$(PDFLATEX) $(MAIN)
	$(PDFLATEX) $(MAIN)

# Bits for the drawings
VPATH := draws:$VPATH

# MetaPost figures
mpfiles = racetrack.mp pentagon.mp
mpsfiles = $(mpfiles:%.mp=%-0.mps)

$(mpsfiles): %-0.mps: %.mp macros.mp
	-find $(<D) -name "$(*F)-[0-9]*.mps" | xargs rm
	-rm $(<D)/"ltx-$(*F).*"
	cd $(<D) && mpost $(<F)
	cd $(<D) && mpost $(<F)
	cd $(<D) && sh ../munge-filenames $(*F)

figures: figures-stamp

figures-stamp: $(mpsfiles)
	touch figures-stamp

